Alternating minimal energy methods for linear systems in higher dimensions. Part I: SPD systems

We introduce a family of numerical algorithms for the solution of linear system in higher dimensions with the matrix and right hand side given and the solution sought in the tensor train format. The proposed methods are rank--adaptive and follow the alternating directions framework, but in contrast to ALS methods, in each iteration a tensor subspace is enlarged by a set of vectors chosen similarly to the steepest descent algorithm. The convergence is analyzed in the presence of approximation errors and the geometrical convergence rate is estimated and related to the one of the steepest descent. The complexity of the presented algorithms is linear in the mode size and dimension and the convergence demonstrated in the numerical experiments is comparable to the one of the DMRG--type algorithm.

==> tikz/ttdef <==
% Rectangle node with diagonal fill
% Author: Mark Wibrow

\makeatletter

% Shape 'rectangle with diagonal fill'
%
% Inherits everything from rectangle except the behind background path.
%
\pgfdeclareshape{rectangle with diagonal fill}
{
    % This bit from \pgflibarayshapes.code.tex
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
   \inheritanchor[from=rectangle]{north}
   \inheritanchor[from=rectangle]{north west}
   \inheritanchor[from=rectangle]{north east}
   \inheritanchor[from=rectangle]{center}
   \inheritanchor[from=rectangle]{west}
   \inheritanchor[from=rectangle]{east}
   \inheritanchor[from=rectangle]{mid}
   \inheritanchor[from=rectangle]{mid west}
   \inheritanchor[from=rectangle]{mid east}
   \inheritanchor[from=rectangle]{base}
   \inheritanchor[from=rectangle]{base west}
   \inheritanchor[from=rectangle]{base east}
   \inheritanchor[from=rectangle]{south}
   \inheritanchor[from=rectangle]{south west}
   \inheritanchor[from=rectangle]{south east}

   \inheritbackgroundpath[from=rectangle]
   \inheritbeforebackgroundpath[from=rectangle]
   \inheritbehindforegroundpath[from=rectangle]
   \inheritforegroundpath[from=rectangle]
   \inheritbeforeforegroundpath[from=rectangle]

  % Now do the background filling.
   \behindbackgroundpath{%
       % \southwest and \northeast defined by rectangle, but
       % (somewhat annoyingly) not \southeast and \northwest
       % so use this workaround.
       \pgfextractx{\pgf@xa}{\southwest}%
       \pgfextracty{\pgf@ya}{\southwest}%
       \pgfextractx{\pgf@xb}{\northeast}%
       \pgfextracty{\pgf@yb}{\northeast}%
       \ifpgf@diagonal@lefttoright
           \def\pgf@diagonal@point@a{\pgfpoint{\pgf@xa}{\pgf@yb}}%
           \def\pgf@diagonal@point@b{\pgfpoint{\pgf@xb}{\pgf@ya}}%
       \else
           \def\pgf@diagonal@point@a{\southwest}%
           \def\pgf@diagonal@point@b{\northeast}%
       \fi
       \pgfpathmoveto{\pgf@diagonal@point@a}%
       \pgfpathlineto{\northeast}%
       \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}%
       \pgfpathclose
       \ifpgf@diagonal@lefttoright
           \color{\pgf@diagonal@top@color}%
       \else
           \color{\pgf@diagonal@bottom@color}%
       \fi
       \pgfusepath{fill}%
       \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}%
       \pgfpathlineto{\southwest}%
       \pgfpathlineto{\pgf@diagonal@point@b}%
       \pgfpathclose
       \ifpgf@diagonal@lefttoright
           \color{\pgf@diagonal@bottom@color}%
       \else
           \color{\pgf@diagonal@top@color}%
       \fi
       \pgfusepath{fill}%
   }
}

\newif\ifpgf@diagonal@lefttoright
\def\pgf@diagonal@top@color{white}
\def\pgf@diagonal@bottom@color{gray!30}

% Use these with PGF
\def\pgfsetdiagonaltopcolor#1{\def\pgf@diagonal@top@color{#1}}%
\def\pgfsetdiagonalbottomcolor#1{\def\pgf@diagonal@bottom@color{#1}}%
\def\pgfsetdiagonallefttoright{\pgf@diagonal@lefttorighttrue}%
\def\pgfsetdiagonalrighttoleft{\pgf@diagonal@lefttorightfalse}%

% Use these with TikZ
\tikzoption{diagonal top color}{\pgfsetdiagonaltopcolor{#1}}
\tikzoption{diagonal bottom color}{\pgfsetdiagonalbottomcolor{#1}}
\tikzoption{diagonal from left to right}[]{\pgfsetdiagonallefttoright}
\tikzoption{diagonal from right to left}[]{\pgfsetdiagonalrighttoleft}
\makeatother
%
% Local definitions
%
\tikzstyle{core}=[rectangle,draw=black,fill=white,thick,minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corel}=[rectangle with diagonal fill, diagonal from left to right, diagonal top color=black!05, diagonal bottom color=white, draw=black, thick,minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corer}=[rectangle with diagonal fill, diagonal from right to left, diagonal top color=black!05, diagonal bottom color=white, draw=black, thick,minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corell}=[rectangle,thick,draw=black,pattern=north west lines,pattern color=black!60, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corerr}=[rectangle,thick,draw=black,pattern=north east lines,pattern color=black!60, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corez}=[rectangle,thick,draw=black,fill=black!10, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corex}=[rectangle,thick,draw=black,fill=black!25, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{corev}=[rectangle,thick,draw=white,fill=white, minimum width=\TIKZcoresize,minimum height=\TIKZcoresize]
\tikzstyle{bond}=[draw]
\tikzstyle{void}=[circle,minimum size=\TIKZlspan]
\endinput

